Automatic Expert Discovery in LLM Upcycling via Sparse Interpolated Mixture-of-Experts

We present Sparse Interpolated Mixture-of-Experts (SIMoE) instruction-tuning, an end-to-end algorithm designed to fine-tune a dense pre-trained Large Language Model (LLM) into a MoE-style model that possesses capabilities in multiple specialized domains. During instruction-tuning, SIMoE automatically identifies multiple specialized experts under a specified sparsity constraint, with each expert representing a structurally sparse subset of the seed LLM's parameters that correspond to domain-specific knowledge within the data. SIMoE simultaneously learns an input-dependent expert merging strategy via a router network, leveraging rich cross-expert knowledge for superior downstream generalization that surpasses existing baselines. Empirically, SIMoE consistently achieves state-of-the-art performance on common instruction-tuning benchmarks while maintaining an optimal performance-compute trade-off compared to all baselines.

==> latex/sections/results/compute.tex <==
\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Method}& \multicolumn{3}{c}{\textbf{Training}} & \multicolumn{2}{c}{\textbf{Inference}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-6}
& \textbf{Memory (G)} & \textbf{Total (B)} & \textbf{Trainable (B)} & \textbf{Total (B)} & \textbf{TFLOPs} \\
\midrule
% Full fine-tuning & & 3.21 & 3.21 & 3.21 & 2.10 \\
SIMoE 3B & 47.24 & 6.08 & & 4.01 & \\
Upcyc./BTX 3B & 65.43 & 11.67 & 11.67 & 11.67 & 3.19 \\
\midrule
% Full fine-tuning & & & & & \\
SIMoE 8B & & & & & \\
Upcyc./BTX 8B & & & & & \\
\bottomrule
\end{tabular}%
}
\caption{\label{tab:train-test-compute}GPU memory requirement for training and inference. Total and Trainable refer to number of model parameters. \chen{flops do not look right, trying other measure that reflect inference speed, possibly token/mins.... anyways I will probably make this into a bar plot.}}
\end{table}
